The incel lexicon: Deciphering the emergent cryptolect of a global misogynistic community

Evolving out of a gender-neutral framing of an involuntary celibate identity, the concept of `incels' has come to refer to an online community of men who bear antipathy towards themselves, women, and society-at-large for their perceived inability to find and maintain sexual relationships. By exploring incel language use on Reddit, a global online message board, we contextualize the incel community's online expressions of misogyny and real-world acts of violence perpetrated against women. After assembling around three million comments from incel-themed Reddit channels, we analyze the temporal dynamics of a data driven rank ordering of the glossary of phrases belonging to an emergent incel lexicon. Our study reveals the generation and normalization of an extensive coded misogynist vocabulary in service of the group's identity.

==> correspondence/2021-05-24incel-lexicon-letter.body.tex <==
To the Editors:

We are very pleased to submit our manuscript for your consideration:

\textbf{``Computational timeline reconstruction of the stories surrounding Trump:\\ Story turbulence, narrative control, and collective chronopathy''}\\
(arXiv version:
\url{https://arxiv.org/abs/2008.07301}).

From the paper's abstract:
\begin{enumerate}
\item 
Measuring the specific kind, temporal ordering, diversity, and turnover rate
of stories surrounding any given subject
is essential to 
developing a complete reckoning
of that subject's historical impact.
\item 
Here, we use Twitter as a distributed news and opinion aggregation source
to identify and track the dynamics of
the dominant day-scale stories around Donald Trump,
the 45th President of the United States.
\item 
Working with a data set comprising around 20 billion 1-grams,
we first compare each day's 1-gram and 2-gram usage frequencies
to those of a year before,
to create day- and week-scale timelines for Trump stories
for 2016 onwards.
\item 
We measure Trump's narrative control, the extent to which stories
have been about Trump or put forward by Trump.
\item 
We then quantify story turbulence and
collective chronopathy---the rate at which
a population's stories for a subject seem to change over time.
\item 
We show that 2017 was the most turbulent overall year for Trump.
Story generation slowed dramatically during
the major waves of the COVID-19 pandemic in 2020,
with rapid turnover returning  first with the
Black Lives Matter protests following George Floyd's murder.
\item
We capture the story timeline and quantify the resurgence story turbulence
in the events leading up to and following the 2020 presidential election,
including the debate, Trump's contraction of COVID,
the claims of election fraud,
Siege of Capitol, Trump's ban from Twitter, and Trump's second impeachment.
\item 
For one example, Trump story turnover for 2 months during the COVID-19 pandemic
was on par with that of 3 days in September 2017.
\item 
Our methods may be applied to any well-discussed phenomenon,
and have potential to enable
the computational aspects of journalism, history, and biography.
\end{enumerate}

We emphasize that 
our paper contains both new methods and new observations for and of socio-political phenomena,
and that our techniques can be generalized more broadly to any realm of human behavior
that is popularly discussed online or otherwise.

We introduce a set of new methodologies for analyzing real-time and historical large-scale texts,
allowing for new conceptions of aiding historical analysis through computation means.

Our timeline reconstruction through keyword extraction has great potential for
historians and political scientists in their efforts to understand
``what happened'' which is in part reflected in ``what was talked about''.

We conceive of and
quantify narrative control for Trump, showing marked variation in time and across topics.
The COVID-19 pandemic, for example, has been a time of Trump having
unusually limited narrative control.

We define and
operationalize the sense of time passing for populations---collective chronopathy---and
produce a detailed analysis of how story turbulence around Trump
induces a distortion through nonlinear correlations between the present and the past
(story and memory of story).

Our intention was to conclude the period of analysis through 2020/12/31 or the end of Trump's term,
though a stopping point now remains unclear.
However, the paper is essentially complete as is and we feel can enter
the review process now.

We believe our paper will be of great benefit to a broad academic audience
and of interest to the general public.

We look forward to hearing of your decision.

Yours sincerely and on behalf of the manuscript's authors,


==> correspondence/general.settings.tex <==
\usepackage{graphicx}
\usepackage{url}
\usepackage{hyperref}

\usepackage{marvosym}

\usepackage[svgnames]{xcolor}
\definecolor{lightgrey}{rgb}{0.7,0.7,0.7}
\definecolor{grey}{rgb}{0.5,0.5,0.5}


\setlength{\oddsidemargin}{20pt}
\setlength{\topmargin}{-20pt}
\setlength{\textwidth}{5in}
\setlength{\textheight}{600pt}

\setlength{\parindent}{0pt}
\setlength{\parskip}{10pt}

\pagestyle{plain}

\renewcommand{\baselinestretch}{1.1}

\newcommand{\etal}{\textit{et al.}}

